Container: Context Aggregation Network

Convolutional neural networks (CNNs) are ubiquitous in computer vision, with a myriad of effective and efficient variations. Recently, Transformers -- originally introduced in natural language processing -- have been increasingly adopted in computer vision. While early adopters continue to employ CNN backbones, the latest networks are end-to-end CNN-free Transformer solutions. A recent surprising finding shows that a simple MLP based solution without any traditional convolutional or Transformer components can produce effective visual representations. While CNNs, Transformers and MLP-Mixers may be considered as completely disparate architectures, we provide a unified view showing that they are in fact special cases of a more general method to aggregate spatial context in a neural network stack. We present the \model (CONText AggregatIon NEtwoRk), a general-purpose building block for multi-head context aggregation that can exploit long-range interactions \emph{a la} Transformers while still exploiting the inductive bias of the local convolution operation leading to faster convergence speeds, often seen in CNNs. In contrast to Transformer-based methods that do not scale well to downstream tasks that rely on larger input image resolutions, our efficient network, named \modellight, can be employed in object detection and instance segmentation networks such as DETR, RetinaNet and Mask-RCNN to obtain an impressive detection mAP of 38.9, 43.8, 45.1 and mask mAP of 41.3, providing large improvements of 6.6, 7.3, 6.9 and 6.6 pts respectively, compared to a ResNet-50 backbone with a comparable compute and parameter size. Our method also achieves promising results on self-supervised learning compared to DeiT on the DINO framework. Code is released at \url{https://github.com/allenai/container}.

==> get_flops.tex <==
class Attention(nn.Module):
    def __init__(self, dim, num_heads=8, qkv_bias=False, qk_scale=None, attn_drop=0., proj_drop=0., seq_l=196):
    
       super().__init__()
        self.num_heads = num_heads
        head_dim = dim // num_heads
        self.scale = qk_scale or head_dim ** -0.5

        self.qkv = nn.Linear(dim, dim * 3, bias=qkv_bias)
        
        #Uncomment this line for Container-PAM
        #self.static_a = 
        #nn.Parameter(torch.Tensor(1, num_heads, 1 + seq_l , 1 + seq_l))
        #trunc_normal_(self.static_a)
        
        self.attn_drop = nn.Dropout(attn_drop)
        self.proj = nn.Linear(dim, dim)
        self.proj_drop = nn.Dropout(proj_drop)

    def forward(self, x):
        B, N, C = x.shape
        qkv = self.qkv(x).reshape(B, N, 3, self.num_heads, C // self.num_heads).permute(2, 0, 3, 1, 4)
        q, k, v = qkv[0], qkv[1], qkv[2]   

        attn = (q @ k.transpose(-2, -1)) * self.scale
        attn = attn.softmax(dim=-1)
        
        #Uncomment this line for Container-PAM
        #attn = attn + self.static_a
        
        attn = self.attn_drop(attn)

        x = (attn @ v).transpose(1, 2).reshape(B, N, C)
        x = self.proj(x)
        x = self.proj_drop(x)
        return x

==> macros/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> macros/space_saver.tex <==
% Some illegal space-saving macros
\parskip=5pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies


\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}
{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}

\newlength{\eqnReduceTop}
\newlength{\eqnReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}


%
\setlength{\subsectionReduceTop}{-0.09in}
\setlength{\subsectionReduceBot}{-0.09in}
\setlength{\sectionReduceTop}{-0.12in}
\setlength{\sectionReduceBot}{-0.12in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.05in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\eqnReduceTop}{-0.05in}
\setlength{\eqnReduceBot}{-0.05in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.14in}
\setlength{\captionReduceBot}{-0.12in}
%\setlength{\captionReduceBot}{-0.15in}

\newcommand{\csection}[1]{\vspace{\sectionReduceTop}\section{#1}\vspace{\sectionReduceBot}}
\newcommand{\csubsection}[1]{\vspace{\subsectionReduceTop}\subsection{#1}\vspace{\subsectionReduceBot}}
\newcommand{\csubsubsection}[1]{\vspace{\subsubsectionReduceTop}\subsubsection{#1}\vspace{\subsubsectionReduceBot}}
\newcommand{\cabstract}[1]{\vspace{\abstractReduceTop}\begin{abstract}#1\end{abstract}\vspace{\abstractReduceBot}}


\setlength{\abovecaptionskip}{6pt plus 0pt minus 0pt}
\setlength{\textfloatsep}{12pt plus 0pt minus 0pt}

\setlength{\floatsep}{15pt plus 0pt minus 0pt}

==> sections/3_approach_old.tex <==
\section{Methods}
\subsection{Overview}
We first revisit the definition of transformer, depth-wise convolution and MLP-Mixer in section~\ref{section:revist}. Then, we provide a unified view of transformer with depth-wise convolution in section ~\ref{section:depthwise} and MLP-Mixer in section~\ref{section:MLP} by linking them using affinity matrix. We show that seemingly different architectures are exploring similar architecture. Built on the unified view, we proposed a fast convergence and high accuracy \pac whose building block use mixture of dynamic and static affinity matrix in section ~\ref{section:pacnet}. Then \paclight provide a simple solution for efficient backbone design by combing the pros of local and global information aggregation and lightweight computation given high resolution input in section~\ref{section:paclight}. 
\subsection{Revisit Transformer, Depthwise Convolution and MLP-Mixer}
\label{section:revist}
Transformer consists of multi-head self-attention module(MHSA) followed by feedforward module(FFN). For MHSA, given flattened visual feature $x  \in \mathbb{R}^{(HW) \times C }$, where $HW$ represent the number of spatial position while $C$ stands for the channel number, $x$ will be projected into $Q  \in \mathbb{R}^{(HW) \times C }$, $K  \in \mathbb{R}^{(HW) \times C }$ and $V  \in \mathbb{R}^{(HW) \times C }$ space using linear transform. Q, K and V stands for Query, Key and Value feature. After getting Key, Query and Value, Key and Query will be multiplied and normalized by softmax to generate an affinity matrix $A \in \mathbb{R}^{(HW) \times (HW) }$. $A_{ij}$ represent the attention weight between $i_{th}$ Query $Q_i$ and $j_{th}$ Key $K_j$. The dot product equation is denoted below :
\begin{align}
    A &= \operatorname{Softmax}(\frac{QK^{T}}{\sqrt{d}}), \label{eq:affinity}
\end{align}
$d$ stands for the number of channel. It will be divided by $QK^T$ to generate a better attention distribution. The affinity matrix in transformer is dynamically generated to reveal the relationship between each query and key. After getting affinity matrix A, A will multiply with V to generate the updated feature for each query. 
\begin{align}
    x &= x + WAV, \label{eq:residual}
\end{align}
Previous discussed self attention is called single-head self-attention. To increase the attention diversity, MHSA further split Q, K and V into different group and perform multiple self attention in parallel and concatenate the updated feature of each head. For multi-head self-attention, the dynamically generated affinity matrix $A \in \mathbb{R}^{h \times (HW) \times (HW)}$, compared with single-head version, the affinity matrix is a three dimensional tensor whose first dimension h stands for the number of heads in transformer. $A_{h} \in \mathbb{R}^{h \times (HW) \times (HW)}$ stands for the dynamically generated affinity matrix in $h_{th}$ head. The MHSA has been denoted by the following equation:

\begin{align}
    A_i &= \operatorname{Softmax}(\frac{Q_i K_i^{T}}{\sqrt{d_h}}), \\
    x = &x + W\operatorname{Concat(A_1 V_1, ...,  A_h V_h)}
\end{align}

Convolution is an important inductive bias in computer vision which use shift-invariant kernel to aggregation local information. Thanks to the local information and weight sharing, CNN has achieved success in many computer vision and NLP application with high accuracy and good computation efficiency. In this work, we mainly focus a special form of convolution, namely, depth-wise convolution. Naive convolution will fuse information from both local and channel dimension which will result in huge computation cost. Group convolution split channel into groups and perform multiple convolution kernel in parallel to reduce the computation and parameters. Depth-wise can be seen as an extreme version of group convolution whose group size equal to input channel dimension. Given input $x  \in \mathbb{R}^{(HW) \times C }$. We will reshape x into $x_r  \in \mathbb{R}^{C \times H \times W }$. Thus the $x_r$ contain neighbour information. Given $x_r$, convolution will use a shift-invariant kernel $K \in \mathbb{R}^{C_{in} \times C_{out} \times k \times k}$ to convolve feature and output a new feature map which contain local information. Group convolution use kernel $K \in \mathbb{R}^{C_{in} \times \frac{C_{out}}{G}  \times k \times k}$ to convolve with input feature, where G is the number of groups. Depthwise convolution use kernel $K \in \mathbb{R}^{C_{in} \times 1  \times k \times k}$ to convolve with input feature $x_r$. In the discussion, we make padding equal to $\frac{k-1}{2}$ and stride is set to 1 by default. This setting will make input and output feature map share the same spatial resolution. We make connection between transformer and depthwise convolution under the default setting. The convolution operator can be written into the following equation:
\begin{align}
    x_r &= x_r + K \circledast x_r, \label{eq:conv1}
\end{align}
Replacing naive convolution with group convolution and depth-wise convolution can make neural network learn better feature and reduce computation burdens. 

MLP-Mixer propose to use transposed MLP for spatial information fusion. We omit the discuss of the second MLP layer as it is same as FFN layer in transformer. The transposed MLP can be written in the following equation:

\begin{align}
    x &= x + (x^T W_{MLP})^T, \label{eq:residual}
\end{align}

T represent transpose operator. $W_{MLP} \in \mathbb{R}^{HW \times HW}$ stands for the weight of MLP layer. 

\subsection{Unifying View for Transformer and Depthwise Convolution}
\label{section:depthwise}
As transformer and convolution capture long range and short range information, how to combine them for efficient learning has been a hot topic. Concurrent to our work, many research naively cascade convolution and transformer and observe gains in performance. Different from them, we provide a unified view of transformer and convolution and write them into a unified equation. 
Starting from depthwise convolution with default padding and stride described in previous section, we rewrite equation \ref{eq:conv1} into the following equation:
\begin{align}
    x &= x + \operatorname{Concat}(B_c x_c), \label{eq:conv2}
\end{align}
We describe the difference between equation~\ref{eq:conv1} and~\ref{eq:conv2} below. The input and output tensor in equation~\ref{eq:conv1} and~\ref{eq:conv2} is $x_r  \in \mathbb{R}^{C \times H \times W }$ and $x  \in \mathbb{R}^{(HW) \times C }$m respectively. Equation~\ref{eq:conv1} use convolution operator, while equation~\ref{eq:conv2} utilize matrix multiplication. $B \in \mathbb{R}^{C_{in} \times (HW) \times (HW)}$ where $C_{in}$ stands for the input channel dimension similar as original convolution definition. B matrix in equation~\ref{eq:conv2} can be seen as an affinity matrix defined in ~\ref{eq:affinity}. $B_{cij}$ stands for the information node j will be propogated to node i in channel c. $i_h,i_w,j_h,j_w$ stands for the two dimensional index of $i, j$. 
The weight in affinity matrix B can be written below:
\begin{align}
    B_{cij} = \left\{
        \begin{array}{ll}
            K[c:0:\rvert i_h-j_h \lvert:\rvert i_w-j_w \lvert] \\ \quad \lvert i_h-j_h \rvert \leq \frac{k-1}{2} \ \text{and}  \ \lvert i_w-j_w \rvert \leq \frac{k-1}{2}\\
            0 \\ \quad \lvert i_h-j_h \rvert > \frac{k-1}{2} \ \text{or}  \ \lvert i_w-j_w \rvert > \frac{k-1}{2}
        \end{array}
    \right., \label{eq:static}
\end{align}
Equation \ref{eq:static} change the depthwise convolution operator with kernel K into a pure matrix multiplication operator which is denoted in equation~\ref{eq:conv2} with affinity matrix B. Motivated by the design of transformer, we add to linear projector V and W and result into the following equation:
\begin{align}
    x &= x + WBVx, \label{eq:conv3}
\end{align}
Given input feature x, we will add a linear layer to transform x input Value then matrix B will perform local information aggregation, after local information aggregation, W will add another linear transformation to project feature into a new space.
After arriving at equation ~\ref{eq:conv3}, we can find out that depth-wise convolution can be seen as special form of affinity matrix in equation~\ref{eq:residual}. Different from transformer which dynamically generate affinity matrix using key and query, depth-wise convolution can be seen as a static generated affinity matrix where only key belong to the neighbour of query will have an attention weight which is a predefined learnable parameter and shared for key and query with same relative position. 

\subsection{Unifying View for Transformer and MLP-Mixer}
\label{section:MLP}
Transformer use dynamically generated affinity matrix for information aggregation. MLP-Mixer use transposed MLP for spatial information aggregation. The seemingly different approach can be unifed by affinity matrix. We start with single head transformer which is shown below:

\begin{align}
    x &= x + WAV, \label{eq:residual}
\end{align}


where $A \in \mathbb{R}^{HW \times HW}$. 
We add two linear transformer into MLP-Mixer which project the input x into Value, and then perform transposed MLP and then perform fusion which is denoted below:

\begin{align}
    x &= x + W(V^T W_{MLP})^T ,\\
    x &= x + WW_{MLP}V , \label{eq:mixer}
\end{align}

By comparing equation \ref{eq:residual} and \ref{eq:mixer}, we find that both $W_{MLP}$ and dynamical affinity matrix A can be seen as a information aggregation module. For $i_{th}$ query and $j_{th}$ key, the aggregation weight is  $W_{MLP}_{ij}$ and $A_{ij}$. Thus we show the transposed MLP in MLP-Mixer can be seen as a static affinity matrix transformer with head dimension equal to $C$. There is only 1 head in MLP-Mixer. Motivated by multi-head transformer design, we augment MLP-Mixer with Multi-head mechanism and name it as Multi-head MLP-Mixer. Another difference between transformer perform softmax normalization over the affinity matrix while MLP-Mixer do not. In the experiment session, we show the effects of softmax normalization, multi-head mechanism on MLP-Mixer. From the analysis of previous session, both MLP-Mixer and Depthwise convolution use static affinity matrix for information aggregation. Depthwise convolution share attention weight for the same relative position while MLP-Mixer do not have any weight sharing mechanism. 

The weight matrix is transposed MLP is of shape $W_{MLP} \in \mathbb{R}^{HW \times HW}$. From image with high resolution, $HW \times HW$ will be huge parameters and cause over-fitting. Thus will decompose the $W_{MLP}$ into two small matrix $W_{MLP1} \in \mathbb{R}^{HW \times \frac{HW}{Down}}$ and $W_{MLP2} \in \mathbb{R}^{\frac{HW}{Down}\times HW}$. To increase the representation power, we add a $GELU$ non linear layer which is popular in transformer architecture. We denote our new MLP-Mixer below:

\begin{align}
    x &= x + WW_{MLP1} \operatorname{GELU}(W_{MLP2}V) , \label{eq:mixer}
\end{align}

Motivated by multi-head nomencalture in transformer, we call the transformer-motivated MLP-Mixer as Multi-head MLP-Mixer. Give input $x$, it will be split into $n$ heads. The $W_{MLP}$ is not shared for different head. Each head will perform multiplication of value vector with affinity matrix and concatenate the transformed features of $n$ heads. 

\subsection{Peusdo Code implementation from the perspective of Affinity Matrix Generation}
We showcase the pesudo code implementation of depth-wise convolution, transformer and MLP-Mixer under our unified view. We define $x \in \mathbb{R}^{HW \times C}$ to be the input feature. x will be transformed into $K,Q,V \in \mathbb{R}^{HW \times C}$ using linear transform. Then $K,Q,V$ will be split into M heads of feature which is denoted by  $K_m,Q_m,V_m \in \mathbb{R}^{HW \times C/M}$. Different algorithms will generate different affinity matrix $A \in \mathbb{R}^{M \times HW \times HW}$ in which M stands for the indices of head. Feature among each head will communication with each other using the corrposeding affinity matrix $A_m$ and then concatenate and fused with a linear transformation layer. 

We illustrate the affinity matrix generator using the following algorithm below:
\begin{algorithm}[H]
\SetAlgoLined
\KwResult{Affinity  }
 A = Parameter(M, HW, HW); $V_m \in \mathbb{R}^{HW \times C/M}$ \tcp*{Shared for all} \
 $K_m,Q_m \in \mathbb{R}^{HW \times C/M}$; \tcp*{Transformer} \
 $Kernel \in \mathbb{R}^{M \times 1 \times k \times k}$; \tcp*{Depthwise Convolution} \
 $W_{MLP1} \in \mathbb{R}^{M \times HW \times \frac{HW}{D}}$,  $W_{MLP1} \in \mathbb{R}^{M \times \frac{HW}{D} \times HW}$; \tcp*{MLP-Based Methods} \
 
\For{m in range(M)}{
 \For{i in range(HW)}{
   \For{j in range(HW)}{
        \If{transformer}{
            A[m, i, j] = $Q[m, i]^T K[m, j]$ \;
        }
        \If{convolution}{
            i_h, i_w, j_h, j_w = \lfloor {\frac{i}{H}} \rfloor, i - i_h * H, \lfloor {\frac{j}{H}} \rfloor, j - j_h * H \;
            
            \eIf{|i_h-j_h|<=\frac{k-1}{2} and |i_w-j_w|<=\frac{k-1}{2}\;}
            {
             $A[m, i, j] = K[m, 0, i_h - j_h, i_w - j_w]$\;
            }{
             A[m, i, j] = 0\;
            }  
        }
        \If{mlp}{
            A[m, i, j] = (W_{MLP1}W_{MLP2})^T[m, i, j]\;
        }
   }
  }
}
\If{transformer}{
            A = \operatorname{Softmax}(A) \;
            
}
 \caption{Affinity matrix generator. The difference between transformer, depth-wise convolution and MLP-based methods is only on how to generate affinity matrix}
\end{algorithm}

After getting affinity matrix A, each head will perform feature update U according to the following equation:
\begin{align}
    U_m &= A_m V_m , \label{eq:mixer}
\end{align}
The updated feature will be concatenated and fused using a linear transformation layer:
\begin{align}
    x = x + W\operatorname{Concat}(U_0, ..., U_m, ... U_M)
\end{align}
When heads M equal to $C_{in}$ and add relative shared static affinity inductive bias, we can derive the common depth-wise convolution with kernel k, padding equal to $\floor{\frac{k-1}{2}}$ and stride equal to 1. When heads equal to 1, add a GELU non-linear activation function between two MLP during forward computation and static affinity matrix, we can arrive into MLP-Mixer.  

\subsection{Template architecture}
\label{section:template}
Motivated by the network design in previous work cite{ResNet, PVT Net}, our template architecture contain 4 blocks. Different from ViT/DeiT which down-sample image to a low resolution and keep constant, each block in our template architecture will down-sample the image resolution gradually. Gradually down-sampling can keep details of image which is important for downstream tasks like segmentation and object detection. Each block is a cascade of basic module. Each module contain two sub-modules, the first sub-module will propagate spatial information thus we call spatial propagation module, the second sub-module will propagate channel information thus we call channel propagation module. In this paper, channel propagation module is fixed to a 2 layer MLP which was proposed by Transformer\cite{vaswani2017attention}. Designing better spatial propagation module is the main focus of this paper. Given image I, we will extract a $4 \times 4$ patch, and pass through block 1 for B1 layers, then we will extract $2 \times 2$ patch and pass through block 2 for B2 layers, then we will extract $2 \times 2$ patch and pass through block3 for B3 layers, then we will extract $2 \times 2$ patch and pass through block 4 for B4 layers. The feature dimension in each block will be fixed to be the same. The feature input dimension is fixed to be 128, 256, 320 and 512. For \pac, each block contain 2,3,8,3 layers which result into a network contain 22 Million parameter. \paclight adopt the same architecture as \pac and only turn off the dynamic affinity matrix in the first 3 stages. Thus the first stages can be efficiently implemented by depth-wise convolution operator offered by modern deep learning framework. 
\subsection{\pac}
Motivated by the unifed view of presented in the previous session, we run a parallel of transformer and depthwise convolution to aggreagtion local and global feature and result into the following equation:
\begin{align}
    x &= x + W_cBV_cx + W_sAV_sx, 
\end{align}
$W_c, V_c$ is the weight of linear projector in convolution path while $W_s, V_s$ representes the weight of linear projector in self-attention path. By sharing the weight of linear projector, we could merge the previous equation into a compact form denoted below:
\begin{align}
    x &= x + W(B + A)Vx,
\end{align}
B and A stands for the affinity matrix generated from depthwise convolution and self-attention key query. $B + A$ can be seen as a new affinity matrix which is composed of instance dynamically predicted relationship A and dataset level shared relationship B. We then write affinity matrix A into Key Query multiplication form denoted  below:
\begin{align}
    x &= x + W(B + \operatorname{Softmax}(\frac{QK^{T}}{\sqrt{d}}))Vx,
\end{align}
Motivated by linear transformer which remove softmax normalization, we remove the softmax for normalization of key query product and add a new softmax after mixture of static affinity matrix and dynamically generated affinity matrix and result in the following equation:
\begin{align}
    x &= x + W\operatorname{Softmax}(\frac{QK^{T}}{\sqrt{d}} + B)Vx,
\end{align}    
Motivated by dynamic gate proposed by LSTM, we use a simple learnable parameter $\alpha$ and $\beta$ to differtibale mix long range and short range equation.  We name the following equation the unifying equation:
\begin{align}
    x &= x + W\operatorname{Softmax}(\alpha \frac{QK^{T}}{\sqrt{d}} + \beta B)Vx,
\end{align}
Unifying equation define a basic module which can simultaneous learn long range and short range information in one operator and learn the mixture factor $\alpha$ and $\beta$ in a data driven manner. Unifying Module can be a simple drop-in module by inserting into network. The input and output of Unifying Module have the same dimension. 

\subsection{\pac}
\label{section:pacnet}
In this section, we will starting from DeiT and replacing MHSA module with Unify Module proposed in the previous session. DeiT extract non-overlapping patch $16 \times 16$ in the beginning and then stack multiple layers of transformer for feature extractor. Down-sampling image 16 times in the beginning can achieve high accuracy. However, lost of fine details will be detrimental for downstream tasks which require high resolution input like object detection and semantic segmentation. Motivated by previous hierachical design in image processing, instead of downsampling image in the beginning and keep the feature map resolution constant, we progressively downsample the feature and result into a feature pyramid of feature map. We adopt a four block approach. We adopt downsampling 4 for block 1, downsampling 8 for block 2, downsampling 16 for block 3 and downsampling 32 for block 4. Besides, we replace all LayerNorm with BatchNorm which is a common pratice in computer vision tasks. At last, we replace MHSA module with Unify Module and result into UnifyNet. UnifyNet could perform global and local information aggregation simutaneously and learn the mixture of local and global feature from data.  
\subsection{\paclight}
\label{section:paclight}
UnifyNet has quadratic computation complexity which is similar as original transformer. Thus UnifyNet need unafforadble computation and memory cost for high resolution downstream tasks like object detection and semantic segmentaion. To tackle this, we provide a simple solution for modify UnifyNet better for downstream tasks. We observe that high resolution feature map usually focus on local information while for low resolution feature map attention will perform global information reasoning. Thus for high resolution feature map in block1, block2 and block 3. We set their $\alpha$ to 0 and $\beta$ to 1. While for block 4, we set their $\alpha$ to 1 and $\beta$ to 0. By doing this, we observe significant decrease of computation at the cost of slight decrease of classification accuracy and slower convergence speed. 
\subsection{Architecture Detail}

==> sections/3_approach_old2.tex <==

\section{Methodology}

In this section, we first propose a building block -- contextual aggregation with multi-head attention -- for deep neural networks. Then, we revisit three major architectures -- Transformer~\cite{}, depthwise convolution~\cite{} and the recently proposed MLP-Mixer~\cite{}, and show that these architectures can be unified and represented as special cases our proposed building block. In Sec.~\ref{approch:container}, we propose a variation of our building block 

we propose a fast convergence and high accuracy building block, which is a mixture of self-attention and depthwise convolution. In Sec.~\ref{approch:base_container_light}, we present the base architecture, and an efficient and lighter version of our building block, which achieves state-of-the-art performance on various of benchmarks. 

\subsection{Contextual Aggregation for Vision}
\label{approch:context}
Consider an input image $X \in \mathbb{R}^{C \times H \times W}$, where $C$ and $H \times W$ denote the channel and spatial dimension of the input image, respectively. The input image is first flattened to a sequence of tokens $\{X_i \in \mathbb{R}^C \vert i = 1, \ldots, N\}$, where $N = HW$. Existing vision networks stack multiple building blocks with residual connections \cite{he2016deep}, which is defined as
\begin{equation}
    \mathbf{Y} = \mathcal{F}(\mathbf{X},\{\mathbf{W}_i\}) + \mathbf{X}.
\end{equation}
%
Here, $\mathbf{X}$ and $\mathbf{Y}$ are the input and output vectors of the layers considered, and $\mathbf{W}_i$ is the learning parameters. The core of $\mathcal{F}$ is how to aggregate contextual information into current feature. We first define an affinity matrix $\mathcal{A} \in \mathbb{R}^{N \times N}$ that represents how the contextual features can aggregate into each feature. Thus, Eq.1 can be written as:  
\begin{equation}
    \mathbf{Y} = (\mathcal{A} \mathbf{V}) \mathbf{W}_1 + \mathbf{X}, \label{eq:single_affinity}
\end{equation}
where $\mathbf{V} \in \mathbb{R}^{N \times C}$ is transformed from $\mathbf{X}$ with linear projection $\mathbf{V} = \mathbf{X} \mathbf{W}_2$. $\mathbf{W}_1$ and $\mathbf{W}_2$ are the learnable parameters.
$A_{ij}$ is the affinity value between $X_i$ and $X_j$. 
%
Multiplying affinity matrix with $V$ can propagate information from all features according to the affinity value. 

Multi-head attention \cite{vaswani2017attention} is widely used in transformer based architectures \cite{devlin2018bert}. It allows the model to jointly attend to information from different representation subspaces at different positions. [HS: don't mention multi-head yet. Too specific to transformer. Just mention features can grouped into multiple groups.] Following \cite{vaswani2017attention}, we can learn multiple affinity matrix to capture different relationships. Given the chunked feature ${\mathbf{V}}^i$ where $\{\mathbf{V}^i \in \mathbb{R}^{N \times \frac{C}{M}} \vert i=1,\ldots,M\}$ and $M$ is the number of heads. The multi-head version of Eq. 2 is
\begin{equation}
    \mathbf{Y} = \operatorname{Concat}(A_1 \mathbf{V}_1, \ldots, A_M \mathbf{V}_M) \mathbf{W}_2 + \mathbf{X} \label{eq:multi_affinity}
\end{equation}
where $A_m$ stands for the affinity matrix in each head. Features in each head will perform contextual aggregation according to the head-specific affinity matrix $A_m$. Different $A_m$ can capture multi-relationship exist in feature space thus increase the representation power of contextual aggregation compared with single-head version. 
Note that only spatial information is propagated while no cross-channel information exchange happen during contextual aggregation using affinity matrix. \textcolor{red}{Besides, motivated by self-attention design, there is no non-linearity activation function inside contextual aggregation. All non-linearity activation will be placed in Feed-forward module. }
%$W_1$ and $W_2$ can fuse channel information. 

In the following session, we will show that classical operator like Self-Attention, Depth-wise Convolution and recently proposed MLP-Mixer share similar computation stack. The main difference between them is how to generate affinity matrix. 

\subsection{Connecting Self-Attention, Depthwise Convolution and MLP-Mixer}
% \begin{figure*}[t]
%         \begin{center}
%                 \includegraphics[width=\linewidth]{figures/SA_CONV_MLP.png}
%         \end{center}
%         \caption{Contextual learning propagate information from $j_th$ key to $i_th$ query feature according to the affinity matrix in upper left. Popular architecture like self-attention(upper right), depth-wise convolution(bottom left) and MLP-Mixer(bottom right) can be written into a special form of affinity matrix.  Through the affinity matrix view, the difference between different architectures can be better analyzed. Illustration show sinle-head self-attention, single-head depth-wise convolution and single-head MLP for simplicity. \jl{We need a more compact figure. we need also associate this figure with section 3.3 with different alpha and beta value. we also need to show the multi-head concept here.}}
%         \label{fig:vis}
% \end{figure*}

Self-attention \cite{vaswani2017attention}, depthwise convolution \cite{kaiser2017depthwise} and recent proposed MLP-Mixer \cite{tolstikhin2021mlpmixer} are three distinct building blocks that are (or potentially to be) widely used in the vision community. Here, we show that the three distinct building blocks can be represented by our proposed contextual aggregation block. The only difference is how to define their affinity matrices.

\paragraph{Self-Attention.} In self-attention mechanism, the affinity matrix is modelled by the similarity between the projected query-key pairs. With $M$ heads, the affinity matrix in head m $A_m^{sa}$ can be written as
\begin{equation}
    \mathbf{A}_m^{sa} = \operatorname{Softmax}({\mathbf{Q}_m \mathbf{K}_m^{T}} / {\sqrt{{C} / {M}}}),
\end{equation}
where $\mathbf{K}_m, \mathbf{Q}_m$ are the corresponding key, query in head $m$, respectively.
The affinity matrix in self-attention is dynamically generated and can reveal instance level information. However, this introduced quadratic computation complexity which will generate huge computation given high resolution feature map. 

% After generating affinity matrix for all head, we can perform the computation introduced in session ~\ref{approch:context}.  The affinity matrix $A^{sa}$ in self-attention is generated by Key and Query while they are generated from input feature map $f_{1d}$.

% The affinity matrix has a global view which means key and query at all positions can communicate each other. This increase the upper bound performance of self-attention. At the same time, this introduced quadratic computation complexity which will generate huge computation given high resolution feature map. 

\paragraph{Depthwise Convolution.} 
Convolution operator fuses both spatial and channel information in parallel. This is different from the contextual aggregation block defined above. However, depthwise convolution \cite{kaiser2017depthwise} which is a extreme version of group convolution performs disentangled convolution on each channel. Once the number of head from contextual aggregation block is equal to the channel size $C$, we can define the convolutional affinity matrix given the 1-d kernel ${Ker \in \mathbb{R}^{C \times 1 \times k}}$:
%Native convolution fuse both spatial and channel information from defied local neighbour. Thus native convolution is different from the contextual aggregation mechanism using affinity propagation defined above. 
% Depth-wise convolution popularized by MobileNet and Xception cite[] perform disentangled spatial and channel information aggregation and perform spatial and channel fusion in an interleaving manner. 
% For simplicity, we consider the 1-d depth-wise convolution with kernel ${Ker \in \mathbb{R}^{C \times 1 \times k}}$. Then we set the head number of contextual aggregation defied in equation \ref{eq:multi_affinity} to be the same as input channel $C$. The dimension in each head only contain 1 dimensional feature. Then the depth-wise convolution can be reformulated as a contextual aggregation module using the following affinity matrix $A_{mij}^{conv}$:
\begin{align}
    \mathbf{A}_{mij}^{conv} = \left\{
        \begin{array}{ll}
            Ker[m:0:\rvert i-j \lvert]  \quad &\lvert i - j  \rvert \leq k\\\
            0  \quad &\lvert i - j  \rvert > k 
        \end{array}
    \right., \label{eq:static}
\end{align}
where $\mathbf{A}_{mij}$ is the affinity value between $X_i$ and $X_j$ on head $m$. Different from the affinity matrix obtained from self-attention whose value is conditioned on the input feature, the affinity value from convolution is static -- not depends on the input features, sparse -- only define local connections and shared across the affinity matrix. 
% By looping over the affinity matrix indices, we can get $A^{conv} \in \mathbb{R}^{C \times HW \times HW}$. Then
% we can perform depth-wise convolution using the previously defined multi-head contextual aggregation. 
%
% From the previous discussion, we show that \emph{depth-wise convolution is a multi-head contextual aggregation with head equal to $C$ and a special form of affinity matrix $A^{conv}$}. 
% The entry in the affinity matrix is a learn-able parameter shared over the whole dataset instances. 
% After training, the affinity matrix will be static. Due to the static affinity matrix and only access to local information, the upper-bound performance is limited. However, thanks to the carefully designed parameter sharing mechanism for key-query with same relative position, the convergence and data-efficiency of convolution is superior than self-attention. 
% Besides, convolution bias is linear scalable with respective to input resolution. Thus convolution design has been adopted for downstream tasks which require fine details such as, object detection and instance level segmentation. 

\paragraph{MLP-Mixer} 
The recent proposed MLP-Mixer \cite{tolstikhin2021mlpmixer} does not rely on any convolution or self-attention operator and achieves superior performance on image classification tasks. 
The core of MLP-Mixer is the transposed MLP operation,
which can be denoted as $X = X + (V^T W_{MLP})^T$. We can define the affinity matrix as
\begin{align}
    A^{mlp} = (W_{MLP})^T, \label{eq:residual}
\end{align}
where $W_{MLP}$ is the learnable parameters. This simple equation shows the transposed-MLP operator is a contextual aggregation operator on a single feature group with a dense affinity matrix. Comparing with self-attention and depthwise convolution, the transpose-MLP affinity matrix is static, dense and with no parameter sharing. 

% This reveals that transposed-MLP is a \emph{single head contextual aggregation with affinity defined by $A^{mlp}$.}
% The affinity matrix is static after training and shared across all instances. Compared with self-attention, the affinity matrix is single-head and also static. 
% Compared with depth-wise convolution, the affinity matrix do not have parameter sharing mechanism. 
% This makes MLP-Mixer structure need huge parameters $W_{MLP} \in \mathbb{R}^{HW \times HW}$ compared with  $Kernel \in \mathbb{R}^{C_{in} \times 1 \times k \times k}$. 
% This illustrate that MLP-Mixer need fix input resolution while depth-wise convolution can tackle input image with arbitrary resolution. 
% Besides, the parameters size in MLP-Mixer is quadratic with respective to input resolution while the constant in depth-wise convolution.  

% To save parameter, we decompose $W_{MLP}$ into a multiplication of two low rank matrix $W_{MLP1} \in  \mathbb{R}^{HW \times \frac{HW}{D}}$ and $W_{MLP1} \in  \mathbb{R}^{\frac{HW}{D} \times HW}$, where D control the intermediate feature dimension. \jl{we need to move this in the implementation details.}

The above simple unification reveals the similarities and differences between self-attention, depthwise convolution and MLP-Mixer in the view of how to construct affinity matrix. This shed us the light to create powerful and efficient building blocks for vision Task. 

\subsection{Container Block(New Version)}
\begin{align}
    x &= x + W_1\operatorname{Norm}\left(\alpha A(x) + \beta A\right)V,
\end{align}
From the previous analysis, we show that different architecture are performing similar computation stack. The affinity matrix can be static or dynamically generated. Besides, different inductive bias can define different parameter sharing strategy. Motivated by this, we create a more powerful Container module by mixing dynamic and static affinity matrix using learnable parameter. Our container module is defined below:
\begin{align}
    x &= x + W_1\operatorname{Norm}\left(\alpha \overbrace{ A(x)}^{Dynamic} + \beta \overbrace{A}^{Static}\right)V,
\end{align}
$A(x)$ is a type of affinity matrix which is dynamically generated from input $x$. Affinity matrix $A^{sa}$ defined in equation is the most classic dynamic contextual aggregation. $A$ is static and can capture the dataset-level information. Affinity matrix $A^{conv}$ and $A^{mlp}$ defined in equation is the most classic static contextual aggregation. 
\begin{itemize}
    \item $\alpha = 1$, $\beta = 0$, $A(x)=A^{sa}$: Container Block will be Transformer block.
    \item $\alpha = 0$, $\beta = 1$, $A = A^{conv}$, $M=C$: Container Block will be depthwise convolution block.
    \item $\alpha = L$, $\beta = L$, $A(x)=A^{sa}$, $A = A^{mlp}$  Container Block will be fuse dynamic and static information. We call this module Pay Attention to MLP (PAM).
    \item $\alpha = L$, $\beta = L$, $A(x)=A^{sa}$, $A = A^{conv}$  Container Block will be fuse dynamic and static information. Different form PAM, the static affinity matrix contain locality constraint and shift invariance which can better tackle vision task. We call this module Pay Attention to Convolution (PAC). 
\end{itemize}

\subsection{Container Block}
\label{approch:container}

To create a more powerful Container block, we want to best of the both world. We mix dynamic contextual of self-attention and locally constrained contextual of depth-wise convolution with learn-able parameter. Our proposed Containter Block is:
\begin{align}
    x &= x + W_1\operatorname{Softmax}\left(\alpha \frac{QK^{T}}{\sqrt{d}} + \beta B\right)V,
\end{align}



where $Q$, $K$,$V$ and query, key and value respectively. $W$ and $B$ are the learnable parameters and  $\alpha$ and $\beta$ are learned mixture weight that can switch between dynamic contextual and static local contextual in a data driven manner. The container block can approximate self-attention block, local-self attention block, depthwise convolution block with specific $\alpha$, $\beta$ and $B$.
\begin{itemize}
    \item $\alpha = 1$ and $\beta = 0$: Container Block will be Transformer block.
    \item $\alpha = 0$, $\beta = 1$ and $B = A^{conv}$: Container Block will be depthwise convolution block.
    \item $\alpha = 0$, $\beta = 1$ and $B =$ Mask: Container Block will be local-transformer block.
\end{itemize}
\jl{not sure this is the best way to show our proposed container block. We need to show this with a figure. Talk about the merits after that.}

% Main thread : $A^{sa}$ dynamically capture instance level contextual aggregation information. As the contextual  in self-attention is large, it takes a long time for self-attention based contextual aggregation to converge. Besides, the quadratic computation cost is self-attention make is hard to be adopted in object detection and segmentation task which need high resolution for reasonable performance. $A^{sa}$ static and constrained local thus performance is limited, fast convergence, high resolution scalable, parameter sharing. $A^{mlp}$ high capacity a weight for all interaction pair, lack of inductive bias make it hard for efficient learning, unable for varied resolution. 

% We mix dynamic contextual of self-attention and locally constrained contextual of depth-wise convolution with learn-able parameter $\alpha$ and $\beta$. We name our module \pac. \pac can switch between dynamic contextual and static local contextual in a data driven manner. 


% \begin{figure*}[t]
%         \begin{center}
%                 \includegraphics[width=\linewidth]{figures/PACNET.png}
%         \end{center}
%         \caption{Affinity matrix for \pac which mix static convolution bias with dynamically generated affinity using key query interaction in 1-d case.  }
%         \label{fig:vis}
% \end{figure*}


% \begin{align}
%     A_m = \alpha A_m^{sa} + \beta A_m^{conv}, \label{eq:residual}
% \end{align}


\subsection{Base Architecture and Container-Light}
\label{approch:base_container_light}
\paragraph{Base Architecture}

To verify the learning ability of different contextual module in a fair way, we use the basic network architecture and only replace the contextual module with affinity generated by self-attention, depth-wise convolution, MLP, \pac and \paclight.

Motivated by the network design in previous work \cite{ResNet, PVT Net}, our base architecture contains 4 blocks. Different from ViT/DeiT which down-sample image to a low resolution and keep the feature map resolution to be constant, each block in our template architecture down-samples the image resolution gradually. Gradually down-sampling can keep details of image, which is important for downstream tasks like segmentation and object detection. Each block is a cascade of basic module. Each module contain two sub-modules, the first sub-module will propagate spatial information thus we call spatial propagation module, the second sub-module will propagate channel information thus we call channel propagation module. In this paper, channel propagation module is fixed to a 2 layer MLP which was proposed by Transformer\cite{vaswani2017attention}. Designing better spatial propagation module is the main focus of this paper. Given image I, we will extract a $4 \times 4$ patch, and pass through block 1 for B1 layers, then we will extract $2 \times 2$ patch and pass through block 2 for B2 layers, then we will extract $2 \times 2$ patch and pass through block3 for B3 layers, then we will extract $2 \times 2$ patch and pass through block 4 for B4 layers. The feature dimension in each block will be fixed to be the same. The feature input dimension is fixed to be 128, 256, 320 and 512. For \pac, each block contain 2,3,8,3 layers which result into a network contain 22 Million parameter. \paclight adopt the same architecture as \pac and only turn off the dynamic affinity matrix in the first 3 stages. Thus the first stages can be efficiently implemented by depth-wise convolution operator offered by modern deep learning framework. 

\jl{show the backbone figure and explain it in words. }

\paragraph{Container-Light}
For computation efficiency and visual backbone deisgn, we truncate the dynamic affinity in \pac in high resolution feature and only keep the mixture of dynamic and local static mechanim in the low resolution feature map and result in \paclight. 

UnifyNet has quadratic computation complexity which is similar as original transformer. Thus UnifyNet need unafforadble computation and memory cost for high resolution downstream tasks like object detection and semantic segmentaion. To tackle this, we provide a simple solution for modify UnifyNet better for downstream tasks. We observe that high resolution feature map usually focus on local information while for low resolution feature map attention will perform global information reasoning. Thus for high resolution feature map in block1, block2 and block 3. We set their $\alpha$ to 0 and $\beta$ to 1. While for block 4, we set their $\alpha$ to 1 and $\beta$ to 0. By doing this, we observe significant decrease of computation at the cost of slight decrease of classification accuracy and slower convergence speed. 

\begin{align}
    A_m^{\paclight} = \left\{
        \begin{array}{ll}
            A_m^{conv}  \quad  &Down = 4, 8, 16\\\
            \alpha A_m^{sa} + \beta A_m^{conv}  \quad  &Down = 32 
        \end{array}
    \right., \label{eq:static}
\end{align}


%-, native convolution fuse information from both spatial and channel in parallel. While our framework (self-attention maybe?) fuse the spatial and channel information in a step-wise manner (iteratively).

%- We consider the highly efficient depth-wise convolution, which maintain the channel-wise disparity in our framework.

%- For simplicity, Given an 2D depthwise convolution Kernel $Kernel \in \mathbb{R}^{C_{in} \times 1  \times k \times k}$. When the number of head is equal to C, The affinity matrix $A^{conv} \in \mathbb{R}^{M \times N \times N}$ can be written as

%\begin{align}
%    A_{mij}^{conv} = \left\{
%        \begin{array}{ll}
%            K[m:0:\rvert i_h-j_h \lvert:\rvert i_w-j_w \lvert] \\ \quad \lvert i_h-j_h \rvert \leq \frac{k-1}{2} \ \text{and}  \ \lvert i_w-j_w \rvert \leq \frac{k-1}{2}\\
%            0 \\ \quad \lvert i_h-j_h \rvert > \frac{k-1}{2} \ \text{or}  \ \lvert i_w-j_w \rvert > \frac{k-1}{2}
%        \end{array}
%    \right., \label{eq:static}
%\end{align}

%$A_{mij}$ stands for the affinity matrix of head m, the affinity value between ith Query and jth Key. $i_h,i_w,j_h,j_w$ stands for the two dimension coordinate while i, h is the indices in one dimension coordinate. After getting affinity matrix $A^{conv}$, we can perform contextual learning using equation introduced in session \ref{approch:context}. The computation between convolution operator and affinity matrix differences in the following. The input feature for convolution is two dimensional feature $f_{2d}$. $f_{2d}$ is good for local neighbour extraction operator. The input feature for affinity matrix approach is $f_{1d}$. $f_{1d}$ is good when the key for query is the same. \textcolor{red}{the sentence is hard to understand. If you do not understand the true meaning, please contact me.}. From the previous discussion, we show that depth-wise convolution construct a special form of affinity matrix. The entry in the affinity matrix is a learn-able parameter shared over the whole dataset instances. After training, the affinity matrix will be static. Due to the static affinity matrix and only access to local information, the upper-bound performance is limited. However, thanks to the carefully designed parameter sharing mechanism for key-query with same relative position, the convergence and data-efficiency of convolution is superior than self-attention. 


% Thanks to the local information and weight sharing, CNN has achieved success in many computer vision and NLP application with high accuracy and good computation efficiency. 
% In this work, we mainly focus a special form of convolution, namely, depth-wise convolution. Naive convolution will fuse information from both local and channel dimension which will result in huge computation cost. 
% Group convolution split channel into groups and perform multiple convolution kernel in parallel to reduce the computation and parameters. Depth-wise can be seen as an extreme version of group convolution whose group size equal to input channel dimension. 
% Given input $f_{2d}  \in \mathbb{R}^{ C \times H \times W }$, convolution will use a shift-invariant kernel $Kernel \in \mathbb{R}^{C_{in} \times C_{out} \times k \times k}$ to convolve feature and output a new feature map which contain local information. Group convolution use kernel $K \in \mathbb{R}^{C_{in} \times \frac{C_{out}}{G}  \times k \times k}$ to convolve with input feature, where G is the number of groups. 
% Depthwise convolution use kernel $Kernel \in \mathbb{R}^{C_{in} \times 1  \times k \times k}$ to convolve with input feature $f_{2d}$. 
% In the discussion, we make padding equal to $\frac{k-1}{2}$ and stride is set to 1 by default. This setting will make input and output feature map share the same spatial resolution. 
% We make connection between transformer and depthwise convolution under the default setting. 
% The convolution operator can be written into the following equation:
% \begin{align}
%     f_{2d} &= f_{2d} + Kernel \circledast f_{2d}, \label{eq:conv1}
% \end{align}
% To make connection with contextual learning in section ~\ref{approch:context}, we add to $1 \times 1$ convolution whose kernel are $W1 \in \mathbb{R}^{C \times C \times 1 \times 1}$ and $W2 \in \mathbb{R}^{C \times C \times 1 \times 1}$. $W_1$ will transformed $f_{2d}$ into a value space, then convolve features at value space with $Kernel$ to propagate spatial information, then $W_2$ will cross-channel information exchange after local spatial aggregation. 
% After introducing depth-wise convolution, we introduce Multi-head depth-wise Convolution(MHDC). Different from depth-wise convolution whose $kernel \in \mathbb{R}^{C_{in} \times 1  \times k \times k}$, it means each channel aggregate different local information in depth-wise convolution. Different from depth-wise convolution, MHDC will share the kernel in neighbour channel. Given M-heads MHDC, the $kernel \in \mathbb{R}^{M \times 1  \times k \times k}$. It will share the spatial information aggregation for every $\frac{C_{in}}{M}$ channels. MHDC can use the default depth-wise convolution interface provide by current deep learning framework like tensorflow and pytorch. The pytorch-style pseudo-code of MHDC is denoted below:

% MHDC can be rewritten as a special form of affinity matrix $A^{conv} \in \mathbb{R}^{M \times HW \times HW}$. The convert between the $Kernel$ in MHDC and $A^{conv}$ is denoted below:
% \begin{align}
%     A_{mij}^{conv} = \left\{
%         \begin{array}{ll}
%             K[m:0:\rvert i_h-j_h \lvert:\rvert i_w-j_w \lvert] \\ \quad \lvert i_h-j_h \rvert \leq \frac{k-1}{2} \ \text{and}  \ \lvert i_w-j_w \rvert \leq \frac{k-1}{2}\\
%             0 \\ \quad \lvert i_h-j_h \rvert > \frac{k-1}{2} \ \text{or}  \ \lvert i_w-j_w \rvert > \frac{k-1}{2}
%         \end{array}
%     \right., \label{eq:static}
% \end{align}
% $A_{mij}$ stands for the affinity matrix of head m, the affinity value between ith Query and jth Key. $i_h,i_w,j_h,j_w$ stands for the two dimension coordinate while i, h is the indices in one dimension coordinate. After getting affinity matrix $A^{conv}$, we can perform contextual learning using equation introduced in session \ref{approch:context}. The computation between convolution operator and affinity matrix differences in the following. The input feature for convolution is two dimensional feature $f_{2d}$. $f_{2d}$ is good for local neighbour extraction operator. The input feature for affinity matrix approach is $f_{1d}$. $f_{1d}$ is good when the key for query is the same. \textcolor{red}{the sentence is hard to understand. If you do not understand the true meaning, please contact me.}. From the previous discussion, we show that depth-wise convolution construct a special form of affinity matrix. The entry in the affinity matrix is a learn-able parameter shared over the whole dataset instances. After training, the affinity matrix will be static. Due to the static affinity matrix and only access to local information, the upper-bound performance is limited. However, thanks to the carefully designed parameter sharing mechanism for key-query with same relative position, the convergence and data-efficiency of convolution is superior than self-attention. 


%\paragraph{Affinity matrix in MLP-Mixer}
%MLP-Mixer propose to use transposed MLP for spatial information fusion. We omit the discuss of the second MLP layer as it is same as FFN layer in transformer. The transposed MLP can be written in the following equation:

%\begin{align}
%    f_{1d} = f_{1d} + (f_{1d}^T W_{MLP})^T, \label{eq:residual}
%\end{align}

%T represent transpose operator. $W_{MLP} \in \mathbb{R}^{HW \times HW}$ stands for the weight of MLP layer. 
%We introduce $W1 \in \mathbb{R}^{C \times C}$ and $W2 \in \mathbb{R}^{C \times C}$. $W1$ will transform $f_{1d}$ into value space, then transposed MLP will propagate information through spatial dimension without cross-channel information exchange. At last $W_2$ will perform channel information fusion. We denote the process below:
%\begin{align}
%    f_{1d} = f_{1d} + ((f_{1d} W1)^T W_{MLP})^T W_2, \label{eq:residual}
%\end{align}
%According to the matrix transpose rule, we can rewrite the previous equation below:
%\begin{align}
%    f_{1d} &= f_{1d} + (W_{MLP})^T (f_{1d} W1) W_2, \label{eq:residual}
%\end{align}
%By comparing with single head contexual learning in equation 2, 3, we can conclude that:
%\begin{align}
%    A^{mlp} = (W_{MLP})^T, \label{eq:residual}
%\end{align}
%This implies that transposed MLP in MLP-Mixer use MLP to generate a single-head affinity matrix. The affinity matrix is static after training and shared across all instances. Compared with self-attention, the affinity matrix is single-head and also static. Compared with multi-head depth-wise convolution, the affinity matrix do not have parameter sharing mechanism. This makes MLP-Mixer structure need huge parameters $W_{MLP} \in \mathbb{R}^{HW \times HW}$ compared with  $Kernel \in \mathbb{R}^{C_{in} \times 1 \times k \times k}$. This illustrate that MLP-Mixer need fix input resolution while depth-wise convolution can tackle input image with arbitrary resolution. Besides, the parameters size in MLP-Mixer is quadratic with respective to input resolution while the constant in depth-wise convolution. 
%To solve the large parameter problem in MLP-Mixer, we decompose $W_{MLP}$ into a multiplication of two low rank matrix $W_{MLP1} \in  \mathbb{R}^{HW \times \frac{HW}{D}}$ and $W_{MLP1} \in  \mathbb{R}^{\frac{HW}{D} \times HW}$. 
%\begin{align}
%    f_{1d} &= f_{1d} + (W_{MLP1} W_{MLP2})^T (f_{1d} W1) W_2, \label{eq:residual}
%\end{align}

%\begin{align}
%    f_{1d} &= f_{1d} + W_{MLP2}^T W_{MLP1}^T (f_{1d} W1) W_2, \label{eq:residual}
%\end{align}

%\begin{align}
%    f_{1d} &= f_{1d} + W_{MLP2}^T \operatorname{GELU}(W_{MLP1}^T) (f_{1d} W1) W_2, \label{eq:residual}
%\end{align}
%Multi-head MLP-Mixer 


% \subsection{Pseudo code for Affinity Matrix Generation}

% We illustrate the affinity matrix generator for Self-attention, multi-head depthwise convolution, multi-head MLP:

% \begin{algorithm}[H]
% \SetAlgoLined
% \KwResult{Affinity  }
%  A = Parameter(M, HW, HW); $V_m \in \mathbb{R}^{HW \times C/M}$ \tcp*{Shared for all} \
%  $K_m,Q_m \in \mathbb{R}^{HW \times C/M}$; \tcp*{Transformer} \
%  $Kernel \in \mathbb{R}^{M \times 1 \times k \times k}$; \tcp*{Multi-head Depthwise Convolution} \
%  $W_{MLP1} \in \mathbb{R}^{M \times HW \times \frac{HW}{D}}$,  $W_{MLP1} \in \mathbb{R}^{M \times \frac{HW}{D} \times HW}$; \tcp*{Multi-head Transposed MLP} \
 
% \For{m in range(M)}{
%  \For{i in range(HW)}{
%   \For{j in range(HW)}{
%         \If{transformer}{
%             A[m, i, j] = $Q[m, i]^T K[m, j]$ \;
%         }
%         \If{convolution}{
%             i_h, i_w, j_h, j_w = \lfloor {\frac{i}{H}} \rfloor, i - i_h * H, \lfloor {\frac{j}{H}} \rfloor, j - j_h * H \;
            
%             \eIf{|i_h-j_h|<=\frac{k-1}{2} and |i_w-j_w|<=\frac{k-1}{2}\;}
%             {
%              $A[m, i, j] = K[m, 0, i_h - j_h, i_w - j_w]$\;
%             }{
%              A[m, i, j] = 0\;
%             }  
%         }
%         \If{mlp}{
%             A[m, i, j] = (W_{MLP1}[m, :, :] W_{MLP2}[m, :, :])^T[i, j]\;
%         }
%   }
%   }
% }
% \If{transformer}{
%             $A = \operatorname{Softmax}(A)$ \;
            
% }
%  \caption{Affinity matrix generator. The difference between transformer, depth-wise convolution and MLP-based methods is only on how to generate affinity matrix}
% \end{algorithm}

% \subsection{Mixture of Diverse Affinity Matrix}
% \begin{figure*}[t]
%         \begin{center}
%                 \includegraphics[width=\linewidth]{figures/diverse_affinity.png}
%         \end{center}
%         \caption{On the right side, we illustrate the computation flow in ViT/DeiT. On the left side, we illustrate the computation flow in \pac. The zoom in view show the attention map in ViT/DeiT vs our proposed \pac. As \pac use depth-wise convolution to capture local information while self-attention to capture long range information simultaneously, the attention map \pac can better capture long range information while naive attention map in ViT/DeiT is constrained to a local region. }
%         \label{fig:vis}
% \end{figure*}

% \subsection{Lightweight Mixture of Diverse Affinity Matrix}

% \subsection{Template Network Architecture}

\begin{figure*}[t]
        \begin{center}
                \includegraphics[width=\linewidth]{figures/overall_graph.png}
        \end{center}
        \caption{The template architecture used for validating the effectiveness of different contextual learning module. Our template architecture will gradually down-sample image and contain four stages with different down-sampling rate. Each stage will contain several blocks. Inside each block, input feature will be processed by a context module followed by channel fusion module.  The template architecture will be pretrained on Imagenet using classification tasks. Then, the pretrained weight will transfer to downstream task such as object detection, instance segmentation, and so on. }
        \label{fig:vis}
\end{figure*}


==> sections/7_checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Sec~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please see Sec~\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Provided in the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Training the large neural networks in this paper is very expensive. Given our limited computational resources, we are unfortunately unable to provide error bars for our experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Provided in the supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> tables/stage_ablation.tex <==
\begin{table}
\setlength\tabcolsep{2pt}
    \centering
    \begin{tabular}{|cccc|c|c|c|c|}
        \hline
        Stage-1 & Stage-2 & Stage-3 & Stage-4 & Top-1 Acc & Params &FLOPs & Throughput \\
        \hline
        \checkmark & \checkmark & \checkmark & \checkmark & 83.1 & 22.1M & &\\
         & \checkmark & \checkmark & \checkmark & 83.1 & 21.8M & &\\
         & & \checkmark & \checkmark &83.0 &21.6M & &\\
         & &  & \checkmark &82.0 &20.0M & &\\
        \hline
    \end{tabular}
    \vspace{6mm}
    \caption{Ablation study of turning off dynamic-affinity matrix in each stage. }
    \label{tab:imagenet_ablation}
\end{table}
